Thompson Sampling with Information Relaxation Penalties

We consider a finite-horizon multi-armed bandit (MAB) problem in a Bayesian setting, for which we propose an information relaxation sampling framework. With this framework, we define an intuitive family of control policies that include Thompson sampling (TS) and the Bayesian optimal policy as endpoints. Analogous to TS, which, at each decision epoch pulls an arm that is best with respect to the randomly sampled parameters, our algorithms sample entire future reward realizations and take the corresponding best action. However, this is done in the presence of "penalties" that seek to compensate for the availability of future information. We develop several novel policies and performance bounds for MAB problems that vary in terms of improving performance and increasing computational complexity between the two endpoints. Our policies can be viewed as natural generalizations of TS that simultaneously incorporate knowledge of the time horizon and explicitly consider the exploration-exploitation trade-off. We prove associated structural results on performance bounds and suboptimality gaps. Numerical experiments suggest that this new class of policies perform well, in particular in settings where the finite time horizon introduces significant exploration-exploitation tension into the problem. Finally, inspired by the finite-horizon Gittins index, we propose an index policy that builds on our framework that particularly outperforms the state-of-the-art algorithms in our numerical experiments.

==> tabular_gauss_5arms_asym_shaded.tex <==

\begin{tabular}{ c c c c c c }
 \toprule
\thead{Algorithm} & \thead{Bayesian regret \\ (s.e.)} & \thead{Regret \\ improvement} & \thead{Regret lower \\ bound (s.e.)} & \thead{Bound \\ improvement} & \thead{Run time} \\
 \midrule
 \textsc{TS} & 121.99 (0.615) & 0.0\% & 0.00 (--) & 0.0\% &  34 ms  \\ 
 \textsc{Irs.FH} & 103.03 (0.628) & 15.5\% & 11.75 (0.656) & 16.2\% &  128 ms  \\ 
 \textsc{Irs.V-Zero} & 89.59 (0.690) & 26.6\% & \textbf{38.47} (0.827) & 53.1\% &  7.4 sec  \\ 
 \textsc{Irs.Index} & 100.20 (0.657) & 17.9\% & -- & -- &  12.8 sec  \\ 
 \textsc{Irs.Index*} & \textbf{72.43} (0.866) & 40.6\% & -- & -- &  12.3 sec  \\ 
 \textsc{Bayes-UCB} & 220.66 (1.285) & -80.9\% & -- & -- &  88 ms  \\ 
 \textsc{IDS} & 94.63 (0.817) & 22.4\% & -- & -- &  2.9 sec  \\ 
 \textsc{OGI} & 151.61 (1.030) & -24.3\% & -- & -- &  829 ms  \\ 

 \bottomrule
\end{tabular}

